Formulating Few-shot Fine-tuning Towards Language Model Pre-training: A Pilot Study on Named Entity Recognition

Fine-tuning pre-trained language models has recently become a common practice in building NLP models for various tasks, especially few-shot tasks. We argue that under the few-shot setting, formulating fine-tuning closer to the pre-training objectives shall be able to unleash more benefits from the pre-trained language models. In this work, we take few-shot named entity recognition (NER) for a pilot study, where existing fine-tuning strategies are much different from pre-training. We propose a novel few-shot fine-tuning framework for NER, FFF-NER. Specifically, we introduce three new types of tokens, "is-entity", "which-type" and bracket, so we can formulate the NER fine-tuning as (masked) token prediction or generation, depending on the choice of pre-trained language models. In our experiments, we apply FFF-NER to fine-tune both BERT and BART for few-shot NER on several benchmark datasets and observe significant improvements over existing fine-tuning strategies, including sequence labeling, prototype meta-learning, and prompt-based approaches. We further perform a series of ablation studies, showing few-shot NER performance is strongly correlated with the similarity between fine-tuning and pre-training.

==> tables/genre.tex <==
% \begin{table*}[]
%     \centering
%     \small
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l c c c c c}
%     \toprule
%     Model\textbackslash Dataset & CoNLL2003 & Onto & WNUT 17 & MitMovie & Restaurant  \\
%     \midrule
%     Sequence Labeling BART-base &  &  &  &  &  \\
%     \midrule
%     Sequence Labeling BART-large &  &  &  &  &  \\
%     \midrule
%     xxx@zilong (UniLM base) & 49.06 ($\pm 3.17$) & 61.11 ($\pm 1.08$) & 15.22 ($\pm 3.10$) & 51.88 ($\pm 1.27$) & 44.17 ($\pm 1.95$)  \\
%     \midrule
%     \our-Bart-base$\ssymbol{2}$ & 58.73 ($\pm 1.77$) & 56.12 ($\pm 0.87$) & 26.98 ($\pm 1.64$) & 52.45 ($\pm 2.01$) & 43.34 ($\pm 1.41$)  \\
%     \midrule
%     \our-Bart-large$\ssymbol{2}$ & 71.00 ($\pm 2.67$) & 64.40 ($\pm 2.88$) & 41.65 ($\pm 1.69$) & 53.25 ($\pm 1.99$) & 51.00 ($\pm 1.52$)  \\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{Experiments on N-way 5 shot NER on 5 datasets with sequence denoising pre-training tasks. $\ssymbol{2}$ is a model adapted from GENRE~\cite{DBLP:conf/iclr/CaoI0P21} that falls under our idea of pre-training alignment.}
%     \label{tab:genre}
% \end{table*}
